Fourier-basis Functions to Bridge Augmentation Gap: Rethinking Frequency Augmentation in Image Classification

Computer vision models normally witness degraded performance when deployed in real-world scenarios, due to unexpected changes in inputs that were not accounted for during training. Data augmentation is commonly used to address this issue, as it aims to increase data variety and reduce the distribution gap between training and test data. However, common visual augmentations might not guarantee extensive robustness of computer vision models. In this paper, we propose Auxiliary Fourier-basis Augmentation (AFA), a complementary technique targeting augmentation in the frequency domain and filling the augmentation gap left by visual augmentations. We demonstrate the utility of augmentation via Fourier-basis additive noise in a straightforward and efficient adversarial setting. Our results show that AFA benefits the robustness of models against common corruptions, OOD generalization, and consistency of performance of models against increasing perturbations, with negligible deficit to the standard performance of models. It can be seamlessly integrated with other augmentation techniques to further boost performance. Code and models can be found at: https://github.com/nis-research/afa-augment

==> section/figs/plot_imagenetbenchmark_org.tex <==
%% Creator: Inkscape 1.3 (0e150ed6c4, 2023-07-21), www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'plot_imagenetbenchmark_org_ink.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{500.30627441bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.30594304)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.08912277,0.06363494){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}1\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.14756303,0.06363494){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}2\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.2060033,0.06363494){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}3\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=4]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.26444356,0.06363494){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}4\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=5]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.32288383,0.06363494){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}5\end{tabular}}}}%
    \put(0.15871577,0.05174754){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}Corruption Severity\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=6]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.03626878,0.08568118){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}30\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=7]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.03626878,0.12156216){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}40\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=8]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.03626878,0.15744315){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}50\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=9]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.03626878,0.19332414){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}60\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=10]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.03626878,0.22920512){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}70\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=11]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.03626878,0.26508611){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}80\end{tabular}}}}%
    \put(0.03224135,0.14425978){\rotatebox{90}{\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}Corruption Error\end{tabular}}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=12]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.19685633,0.29035463){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}IN-C\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=13]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.39961591,0.06363494){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}1\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=14]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.45805616,0.06363494){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}2\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=15]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.51649642,0.06363494){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}3\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=16]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.57493667,0.06363494){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}4\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=17]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.63337697,0.06363494){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}5\end{tabular}}}}%
    \put(0.46920888,0.05174754){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}Corruption Severity\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=18]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.5052115,0.29035463){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}IN-$\mathrm{\Bar{C}}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=19]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.71010901,0.06363494){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}1\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=20]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.76854931,0.06363494){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}2\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=21]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.82698956,0.06363494){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}3\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=22]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.88542982,0.06363494){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}4\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=23]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.94387007,0.06363494){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}5\end{tabular}}}}%
    \put(0.77970203,0.05174754){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}Corruption Severity\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=24]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.79143245,0.29035463){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}IN-3DCC\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=25]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.03531503,0.03071561){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}ResNet50\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=26]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.0335503,0.01164218){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}CCT\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=27]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.14452647,0.03071561){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}RN50+PRIME\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=28]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.14452647,0.01164218){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}RN50+PRIME+AFA\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=29]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.28653381,0.03071561){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}CCT+PRIME\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=30]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.28653381,0.01164218){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}CCT+PRIME+AFA\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=31]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.42854114,0.03071561){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}RN50+TA\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=32]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.42854114,0.01164218){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}RN50+TA+AFA\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=33]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.5705485,0.03071561){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}CCT+TA\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=34]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.5705485,0.01164218){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}CCT+TA+AFA\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=35]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.71255586,0.03071561){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}RN50+AugMix\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=36]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.71255586,0.01164218){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}RN50+AugMix+AFA\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=37]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.87798884,0.03071561){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}CCT+AugMix\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=38]{section/figs/plot_imagenetbenchmark_org_ink.pdf}}%
    \put(0.87798884,0.01164218){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\scriptsize\begin{tabular}[t]{l}CCT+AugMix+AFA\end{tabular}}}}%
  \end{picture}%
\endgroup%


==> section/tables/rebuttal.tex <==
\begin{tabular}{ccccccccccHccl}
    & & & \multicolumn{2}{c}{\bfseries IN-C} & \multicolumn{2}{c}{\bfseries IN-$\bar{\textbf{C}}$}& \multicolumn{2}{c}{\bfseries IN-3DCC} & \multicolumn{2}{c}{\bfseries IN-R} & \multicolumn{1}{c}{\bfseries IN-v2} & \multicolumn{2}{c}{\bfseries IN-P} \\
    \bfseries Main & \bfseries Aux & \bfseries \textcolor{gray}{SA ($\uparrow$)} & \bfseries \textcolor{gray}{RA ($\uparrow$)} & \bfseries \textcolor{gray}{mCE ($\downarrow$)} & \bfseries \textcolor{gray}{RA ($\uparrow$)} & \bfseries \textcolor{gray}{mCE ($\downarrow$)} & \bfseries \textcolor{gray}{RA ($\uparrow$)} & \bfseries \textcolor{gray}{mCE ($\downarrow$)} & \bfseries \textcolor{gray}{Acc. ($\uparrow$)} 
    & \bfseries \textcolor{gray}{RMS ($\downarrow$)} 
    & \bfseries \textcolor{gray}{Avg. Acc. ($\uparrow$)} & \bfseries \textcolor{gray}{mFP ($\downarrow$)} & \bfseries \textcolor{gray}{mT5D ($\downarrow$)} \\ \toprule
    APR-SP & \xmark & 71.9 & 42.9 & 72.7 & 45.9 & 72.5 & 39.8 & 78.4 & 34.9 & 17.2 & 67.2 & 60.2 & 75.4 \\
    -      & AFA   & \gn{76.5} & \gn{46.2} & \gn{68.0} & \gn{47.6} & \gn{69.4} & \gn{46.2} & \gn{69.8} & \gn{38.1} & 16.3 & \gn{72.0} & \gn{48.0} & \gn{67.2} \\
    APR-SP & AFA   & \gn{74.4} & \gn{47.6} & \gn{66.7} & \gn{51.4} & \gn{64.9} & \gn{42.6} & \gn{74.6} & \gn{38.7} & 14.2 & \gn{69.3} & \gn{54.9} & \gn{72.6} \\
    \bottomrule
\end{tabular}


==> section/tables/rebuttal_cvt.tex <==
\begin{tabular}{ccccccccc}
\toprule
    & \multicolumn{4}{c}{\bfseries CVT} & \multicolumn{4}{c}{\bfseries ViT} \\
    & \multicolumn{2}{c}{\bfseries C10-C} & \multicolumn{2}{c}{\bfseries C100-C} & \multicolumn{2}{c}{\bfseries C10-C} & \multicolumn{2}{c}{\bfseries C100-C} \\
    \bfseries Auxiliary & \bfseries SA$\uparrow$ & \bfseries RA$\uparrow$ & \bfseries SA$\uparrow$ & \bfseries RA$\uparrow$ & \bfseries SA$\uparrow$ & \bfseries RA$\uparrow$ & \bfseries SA$\uparrow$ & \bfseries RA$\uparrow$ \\ \toprule
    \xmark & 94.31 & 77.02 & 75.53 & 48.25 & 94.46 & 75.97 & 74.26 & 50.88 \\
    AFA   & \gn{94.53} & \gn{87.03} & \gn{76.96} & \gn{60.12} & \gn{94.58} & \gn{86.71} & \gn{75.13} & \gn{58.25} \\ \bottomrule
\end{tabular}

